An Empirical Study of the Generalization Ability of Lidar 3D Object Detectors to Unseen Domains

3D Object Detectors (3D-OD) are crucial for understanding the environment in many robotic tasks, especially autonomous driving. Including 3D information via Lidar sensors improves accuracy greatly. However, such detectors perform poorly on domains they were not trained on, i.e. different locations, sensors, weather, etc., limiting their reliability in safety-critical applications. There exist methods to adapt 3D-ODs to these domains; however, these methods treat 3D-ODs as a black box, neglecting underlying architectural decisions and source-domain training strategies. Instead, we dive deep into the details of 3D-ODs, focusing our efforts on fundamental factors that influence robustness prior to domain adaptation. We systematically investigate four design choices (and the interplay between them) often overlooked in 3D-OD robustness and domain adaptation: architecture, voxel encoding, data augmentations, and anchor strategies. We assess their impact on the robustness of nine state-of-the-art 3D-ODs across six benchmarks encompassing three types of domain gaps - sensor type, weather, and location. Our main findings are: (1) transformer backbones with local point features are more robust than 3D CNNs, (2) test-time anchor size adjustment is crucial for adaptation across geographical locations, significantly boosting scores without retraining, (3) source-domain augmentations allow the model to generalize to low-resolution sensors, and (4) surprisingly, robustness to bad weather is improved when training directly on more clean weather data than on training with bad weather data. We outline our main conclusions and findings to provide practical guidance on developing more robust 3D-ODs.

==> Figures/sensor_gap_models.tex <==
\begin{figure}[t!]
    \input{iccv2023AuthorKit/Figures/sensor_gap_models_tikz}
    \vspace{-1.5em}
    \caption{Benchmarking the OOD and Oracle performances of several 3D detectors on the KITTI dataset with 16 and 32 lines.}
    \label{fig:sensor_gap_models}
    \vspace{-1.5em}
\end{figure}

==> Figures/sensor_gap_models_tikz.tex <==
\begin{tikzpicture}
\begin{axis}[%
width=2.8in,
height=2.3in,
scale only axis,
xticklabel style = {font=\small},
xlabel style={font=\color{white!15!black}, at={(axis description cs:0.5,0.02)}, anchor=north},
xlabel={\small Oracle 3D AP [\%]},
every outer y axis line/.append style={black},
every y tick label/.append style={font=\small \color{black}},
every y tick/.append style={black},
%every minor tick,
yticklabel style={%
	/pgf/number format/.cd,
	fixed,
	fixed zerofill,
	precision=3,
},
ymin=20,
ymax=65,
ytick={20, 25, 30, 35, 40, 45, 50, 55, 60, 65},
yticklabels = {{}, {25}, {30}, {35},{40},{45},{50},{55}, {60}, {65}},
xmin=40,
xmax=70,
xtick={40, 42, 44, 46, 48, 50,52,54,56, 58, 60, 62, 64, 66, 68, 70},
xticklabels = {{}, {42}, {44}, {46}, {48},{50},{52},{54},{56},{58},{60},{62},{64},{66},{68}, {70}},
ylabel style={font=\color{black}, at={(axis description cs:0.1,0.5)}, anchor=south},
ylabel={\small \textcolor{black}{Target 3D AP [\%] (OOD)}},
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left,
xmajorgrids,
ymajorgrids,
legend pos = north west,
legend style={legend cell align=left, align=left, draw=black, {nodes={scale=0.70}}}
]

\addplot [only marks,
scatter src=explicit symbolic,
scatter/classes={a={mark=square*, draw=blue, mark size=2pt, fill=blue}, b={mark=diamond*, draw=red, fill=red, mark size=3pt}, c={mark=square*, draw=red, mark size=2pt, fill=red}, d={mark=diamond*, draw=red, fill=red, mark size=3pt}},
nodes near coords*={\tiny \Label},
visualization depends on={value \thisrow{label} \as \Label},
visualization depends on=\thisrow{alignment} \as \alignment,
every node near coord/.style={anchor=\alignment}]
table[row sep=crcr, meta=class]{
 x   y    label            class   alignment\\
64.9 60.6   PVRCNN             a        -185\\
66.4 58.6   VOTR-TSD           a        90\\
65.2 61.3   VoxelRCNN          a        -160\\
60.4 57.9   VOTR-VoxelRCNN     a        110\\
55.9 51.2   Second             a        90 \\
57.2 52.7   CenterPoint        a        -180 \\ 
51.3 44.1   PointPillars       a        90 \\
62.0 63.1   PointRCNN          a        0 \\
61.0 50.1   PVRCNN-CenterHead  a        90 \\ 
% 58.6 51.4   SecondIoU          a        -180\\
% 57.5 53.3   SecondIoU-Head     a        -90\\
% 58.2 51.4   Second-MultiHead   a        180\\
58.5 35.9   PVRCNN             b        -180\\
59.3 33.9   VOTR-TSD           b        -180\\
57.2 36.0   VoxelRCNN          b        -90\\
50.7 33.7   VOTR-VoxelRCNN     b        -90\\
50.7 28.3   Second             b        -180 \\
49.6 27.4   CenterPoint        b        90 \\ 
40.6 27.7   PointPillars       b        -180 \\
53.3 32.5   PointRCNN          b        90 \\
53.3 23.9  PVRCNN-CenterHead      b        90 \\
% 51.1 30.7   SecondIoU          b        -180\\
% 52.1 31.4   SecondIoU-Head     b        -90\\
% 51.6 28.9   Second-MultiHead   b        180\\
};

\addplot[black] coordinates {(50.7,33.7) (59.3, 33.9 )};
\addplot[black] coordinates {(57.2, 36.0) (58.5, 35.9 )};
\addplot[black] coordinates {(60.4, 57.9) (66.4, 58.6 )};
\addplot[black] coordinates {( 55.9, 51.2) (57.2, 52.7)};
\addplot[black] coordinates {(53.3, 23.9 ) (58.5, 35.9)};
\addplot[black] coordinates {(49.6, 27.4  ) (50.7, 28.3)};
\addplot[black] coordinates {(61.0, 50.1  ) (64.9, 60.6 )};
\addplot[black,domain=30:70, opacity=0.4]{x};
\legend{Kitti-32, Kitti-16}
\end{axis}
\end{tikzpicture}

==> Figures/sensor_gap_vox_size.tex <==
\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.9\linewidth]{iccv2023AuthorKit/Figures/sensor_gap_voxenc.pdf}
    \caption{We investigate the effect of 12 combinations of the voxel height and NPPV on the OOD performance of 3 models across different resolutions. Higher voxel heights correlate with better OOD performance, especially on KITTI-16 and in VOTR-TSD.}
    \label{fig:sensor_gap_vox_size}
    %\vspace{-1em}
\end{figure*}

==> Supp_Figures/gt_sampling_tp_fp.tex <==
\begin{figure*}[t!]
	\centering
	\includegraphics[scale=.15]{Supp_Figures/with_out_gt.png}
	\caption{Number of True Positives and False Positives predicted by PVRCNN for the pedestrian class on KITTI-64 $\rightarrow$ KITTI-16.} 
	\label{gtsampling_tp_fp}
\end{figure*}

==> Supp_Figures/models_location.tex <==
\begin{figure*}[ht!]
     \centering
     \begin{subfigure}[b]{0.27\textwidth}
         \centering
         \includegraphics[width=\textwidth]{iccv2023AuthorKit/Appendix_Figures/supp_scatter1.pdf}
         \caption{Waymo $\rightarrow$ KITTI}
         \label{subfig:WTK}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{iccv2023AuthorKit/Appendix_Figures/supp_scatter3.pdf}
         \caption{Waymo $\rightarrow$ nuScenes}
         \label{subfig:WTN}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.27\textwidth}
         \centering
         \includegraphics[width=\textwidth]{iccv2023AuthorKit/Appendix_Figures/supp_scatter2.pdf}
         \caption{nuScenes $\rightarrow$ KITTI}
         \label{subfig:NTK}
     \end{subfigure}
        \caption{An overview of different arcitecture OOD performance across various geographical locations.}
        \label{fig:three graphs}
\end{figure*}

==> Supp_Tables/multiclass_kitti.tex <==
\begin{table*}[!t]
    \centering
    \adjustbox{width=\linewidth}{\begin{tabular}{c|c|ccc|ccc}
    \hline
        \multirow{2}{*}{Models} & \multirow{2}{*}{Anchors} & \multicolumn{3}{c|}{Waymo} & \multicolumn{3}{c}{Waymo $\rightarrow$ KITTI} \\ 
        ~ & ~ & Vehicle  & Pedestrian & Cyclist & Vehicle  & Pedestrian & Cyclist \\ \hline
        \multirow{2}{*}{Multi-class Training} & Training & 62.77/54.65 & 49.4/41.88 & 53.77/51.73 & 47.80 / 7.88 & 48.23 / 44.82 & 49.50 / 44.77 \\ 
        ~ & Best performing & N/A & N/A & N/A & 79.74 / 64.36 & 51.48 / 49.31 & 60.15 / 55.97 \\ 
        \midrule
        \multirow{2}{*}{Single Class Training} & Training & 66.68/58.31 & 51.42/43.68 & 57.01/54.92 & 52.42 / 12.62 & 45.20 / 42.31 & 50.94 / 44.48 \\ 
        ~ & Best performing & N/A & N/A & N/A & 80.23 / 66.72 & 49.16 / 46.10 & 60.43 / 55.69 \\ \hline
    \end{tabular}}
    \caption{Multiclass vs Singleclass training on Waymo $\rightarrow$ KITTI.}
    \label{tab:multiclass_kitti}
\end{table*}

==> Supp_Tables/multiple_runs.tex <==
\begin{table}[!ht]
    \centering
     \adjustbox{width=\linewidth}{\begin{tabular}{c|ccc|ccc|ccc}
    \hline
        \multirow{2}{*}{Runs} &  \multicolumn{3}{c|}{VoxelRCNN (5) } & \multicolumn{3}{c|}{VOTR-VoxelRCNN (3)} & \multicolumn{3}{c}{VOTR-TSD (5) } \\ 
         & Car  & Ped  & Cyc & Car  & Ped  & Cyc & Car  & Ped  & Cyc \\ 
        \hline
        Paper Run & 7.48 & 20.96 & 0.00 & 19.26 & 26.82 & 2.04 & 26.26 & 26.56 & 4.70  \\ 
        Mean & 8.22 & 20.26 & 0.00 & 20.17 & 27.63 & 1.43 & 27.1 & 26.42 & 4.4 \\ 
        %Std & 4.862235083 & 4.842626354 & 0 & 2.37394889 & 4.221733451 & 1.177794549 & 3.277906344 & 0.8153710812 & 2.183346056 \\ 
        \hline
    \end{tabular}}
    \caption{Results of Multiple Runs on the N$\rightarrow$K benchmark. We report the number of experiments between brackets.}
    \label{tab:multiple_runs}
    \vspace{-1em}
\end{table}

==> Supp_Tables/sensors_model.tex <==
\begin{table*}[!ht]
    \centering
    \adjustbox{width=0.95\textwidth}{\begin{tabular}{c|cccc|cccc|cccc|c}
    \toprule
         \multirow{2}{*}{Method} & \multicolumn{4}{c|}{Car} & \multicolumn{4}{c|}{Ped} & \multicolumn{4}{c|}{Cyclist} & \multirow{2}{*}{mAP} \\ 
        
        ~ & Easy & Mod. & Hard & Mean & Easy & Mod. & Hard & Mean & Easy & Mod. & Hard & Mean & ~ \\
        \midrule
        \multicolumn{14}{c}{KITTI-64} \\
        \midrule
        PointRCNN & 89.64 & 80.55 & 78.03 & 82.74 & 64.93 & 57.64 & 49.84 & 57.47 & 91.25 & 71.35 & 66.77 & 76.46 & 72.22 \\ 
        PointPillars & 87.55 & 75.11 & 70.83 & 77.83 & 46.77 & 43.01 & 40.34 & 43.37 & 61.67 & 43.53 & 40.34 & 48.51 & 56.57 \\ 
        Second & 88.22 & 77.9 & 73.55 & 79.89 & 51 & 45.77 & 43.31 & 46.69 & 67.46 & 49.32 & 47.02 & 54.6 & 60.39 \\ 
        CenterPoint & 83.44 & 75.47 & 73.19 & 77.36 & 59.03 & 53.13 & 49.95 & 54.04 & 71.46 & 54.9 & 51.19 & 59.18 & 63.53 \\ 
        VoxelRCNN & 92.25 & 82.87 & 80.37 & 85.16 & 71.73 & 66.66 & 61.71 & 66.7 & 85.53 & 64.41 & 61.8 & 70.58 & 74.15 \\ 
        VOTR-VoxelRCNNhead & 92.18 & 82.48 & 79.9 & 84.85 & 66.52 & 61.84 & 56.98 & 61.78 & 75.42 & 58.95 & 56.15 & 63.51 & 70.05 \\ 
        PVRCNN & 91.26 & 82.51 & 80.22 & 84.66 & 64.51 & 58.45 & 55.4 & 59.45 & 83.51 & 62.49 & 59.86 & 68.62 & 70.91 \\ 
        PVRCNN Centerhead & 89.22 & 77.66 & 73.04 & 79.97 & 57.66 & 51.82 & 48.15 & 52.54 & 68.44 & 45.83 & 43.46 & 52.58 & 61.7 \\ 
        VOTR-TSD & 88.99 & 82.09 & 79.9 & 83.66 & 58.83 & 55 & 51.63 & 55.15 & 75.67 & 58.28 & 54.37 & 62.78 & 67.2 \\ 
       \midrule
       \multicolumn{14}{c}{KITTI-64 $\rightarrow$ KITTI-32} \\ 
       \midrule
        PointRCNN & 86.13 & 70.24 & 67.73 & 74.7 & 57.85 & 51.99 & 45.75 & 51.86 & 80.6 & 53.21 & 50.76 & 61.52 & 62.7 \\ 
        PointPillars & 81.8 & 67.22 & 62.42 & 70.48 & 39.11 & 35.3 & 33.01 & 35.81 & 35.47 & 21.63 & 20.69 & 25.93 & 44.07 \\ 
        Second & 85.21 & 69.94 & 65.35 & 73.5 & 45.22 & 40.96 & 37.15 & 41.11 & 50.68 & 34.17 & 32.44 & 39.1 & 51.24 \\ 
        CenterPoint & 81.06 & 67.93 & 64.55 & 71.18 & 46.65 & 42.49 & 38.99 & 42.71 & 58.77 & 38.03 & 35.76 & 44.19 & 52.69 \\ 
        VoxelRCNN & 87.9 & 73.63 & 69.33 & 76.96 & 61.53 & 56.71 & 51.88 & 56.71 & 66.37 & 43.25 & 40.91 & 50.18 & 61.28 \\ 
        VOTR-VoxelRCNNhead & 86.11 & 72.39 & 69.63 & 76.05 & 55.06 & 52.06 & 47.74 & 51.62 & 61.17 & 39.65 & 37.31 & 46.04 & 57.9 \\ 
        PVRCNN Centerhead & 85.78 & 67.48 & 60.91 & 71.39 & 49.51 & 44.19 & 40.21 & 44.64 & 48.03 & 28.34 & 26.24 & 34.2 & 50.08 \\ 
        PVRCNN & 88.05 & 74.42 & 70.4 & 77.62 & 59.39 & 54.1 & 48.38 & 53.96 & 64.94 & 44.95 & 41 & 50.3 & 60.63 \\ 
        VOTR-TSD & 86.15 & 72.66 & 70.07 & 76.29 & 54.26 & 49.34 & 45.73 & 49.78 & 64.29 & 43.62 & 41.38 & 49.76 & 58.61 \\ 
       \midrule
       \multicolumn{14}{c}{KITTI-64 $\rightarrow$ KITTI-16} \\ 
       \midrule 
        PointRCNN & 66.59 & 46.55 & 42.07 & 51.74 & 22.69 & 21.68 & 18.72 & 21.03 & 35.3 & 19.52 & 19.32 & 24.71 & 32.49 \\ 
        PointPillars & 67.64 & 48.5 & 43.35 & 53.16 & 23.06 & 20.35 & 18.08 & 20.5 & 12.47 & 7.76 & 7.6 & 9.28 & 27.65 \\ 
        Second & 65.76 & 45.63 & 40.74 & 50.71 & 18.56 & 16.61 & 14.81 & 16.63 & 24.46 & 14.3 & 13.99 & 17.58 & 28.3 \\ 
        CenterPoint & 67.13 & 48.03 & 43.24 & 52.8 & 16.37 & 15.15 & 13.82 & 15.11 & 20.33 & 11.58 & 10.9 & 14.27 & 27.39 \\ 
        VoxelRCNN & 69.63 & 51.54 & 47.17 & 56.11 & 30.23 & 27.43 & 24.06 & 27.24 & 34.69 & 20.2 & 19.03 & 24.64 & 36 \\ 
        VOTR-VoxelRCNNhead & 70.07 & 50.82 & 46.2 & 55.7 & 26.53 & 24.56 & 22.55 & 24.55 & 29.27 & 16.75 & 16.36 & 20.79 & 33.68 \\ 
        PVRCNN & 68 & 49.35 & 44.87 & 54.07 & 30.22 & 27.29 & 23.87 & 27.13 & 37.42 & 21.68 & 19.98 & 26.36 & 35.85 \\ 
        PVRCNN Centerhead & 59.51 & 39.7 & 33.51 & 44.24 & 18.38 & 15.53 & 12.26 & 15.39 & 17.1 & 10.49 & 8.48 & 12.02 & 23.88 \\ 
        VOTR-TSD & 69.28 & 50.97 & 46.59 & 55.61 & 23.92 & 21.55 & 19.66 & 21.71 & 34.62 & 19.33 & 19.19 & 24.38 & 33.9 \\ 
       \midrule
       \multicolumn{14}{c}{Oracle KITTI-32} \\
       \midrule 
        PointRCNN & 88.41 & 74.44 & 72.06 & 78.31 & 55.32 & 50.17 & 44.35 & 49.95 & 77.63 & 52.35 & 48.45 & 59.47 & 62.57 \\ 
        PointPillars & 83.3 & 69.36 & 65.2 & 72.62 & 47.26 & 41.8 & 38.61 & 42.56 & 51.68 & 32.9 & 31.24 & 38.6 & 51.26 \\ 
        Second & 86.85 & 72.91 & 70.07 & 76.61 & 46.94 & 41.08 & 36.28 & 41.43 & 65.3 & 43.14 & 40.77 & 49.74 & 55.93 \\ 
        CenterPoint & 80.65 & 69.87 & 68 & 72.84 & 53.54 & 48.69 & 45.45 & 49.23 & 63.35 & 44.04 & 41 & 49.46 & 57.18 \\ 
        VoxelRCNN & 89.52 & 77.07 & 74.3 & 80.3 & 60.41 & 53.1 & 47.94 & 53.82 & 78.6 & 54.33 & 51.43 & 61.46 & 65.19 \\ 
        PVRCNN & 91.86 & 77.5 & 74.99 & 81.45 & 59.38 & 50.72 & 45.16 & 51.75 & 77.2 & 55.7 & 51.77 & 61.55 & 64.92 \\ 
        VOTR-VoxelRCNNhead & 89 & 74.81 & 72.07 & 78.63 & 47.39 & 41.89 & 37.75 & 42.34 & 76.82 & 53.46 & 50.72 & 60.33 & 60.43 \\ 
        VOTR-TSD & 91.13 & 79.3 & 76.97 & 82.47 & 55.94 & 50.24 & 45.89 & 50.69 & 84.1 & 59.13 & 54.99 & 66.08 & 66.41 \\ 
       \midrule
       \multicolumn{14}{c}{Oracle KITTI-16} \\
       \midrule 
        PointRCNN & 81.2 & 61.05 & 56.8 & 66.35 & 51.31 & 45.25 & 39.75 & 45.44 & 66.86 & 39.72 & 37.6 & 48.06 & 53.28 \\ 
        PointPillars & 78.4 & 59.53 & 56.21 & 64.71 & 40.26 & 36.02 & 33.06 & 36.45 & 28.66 & 17.12 & 15.74 & 20.51 & 40.56 \\ 
        Second & 82.1 & 63.44 & 59.48 & 68.34 & 48.8 & 42.44 & 37.65 & 42.96 & 56.54 & 33.85 & 31.71 & 40.7 & 50.67 \\ 
        CenterPoint & 75.21 & 60.09 & 57.58 & 64.29 & 50.71 & 45.66 & 41.42 & 45.93 & 52.81 & 32.6 & 30.52 & 38.65 & 49.62 \\ 
        VoxelRCNN & 85.44 & 66.64 & 63.28 & 71.79 & 57.22 & 50.44 & 45.25 & 50.97 & 67.26 & 40.6 & 38.51 & 48.79 & 57.18 \\ 
        VOTR-VoxelRCNNhead & 82.82 & 63.86 & 59.03 & 68.57 & 47.67 & 40.92 & 35.66 & 41.42 & 57.37 & 35.4 & 33.36 & 42.04 & 50.68 \\ 
        PVRCNN  & 85.62 & 68.27 & 64.24 & 72.71 & 59.65 & 52.77 & 46.74 & 53.05 & 67.61 & 42.04 & 39.75 & 49.8 & 58.52 \\ 
        PVRCNN Centerhead & 82.29 & 65.85 & 61.5 & 69.88 & 56.71 & 51.72 & 46.02 & 51.48 & 54.18 & 31.77 & 29.59 & 38.51 & 53.29 \\ 
        VOTR-TSD & 85.77 & 69.22 & 66.27 & 73.75 & 60.07 & 52.58 & 47.69 & 53.45 & 68.35 & 43.05 & 40.67 & 50.69 & 59.3 \\ \hline
    \end{tabular}}
    \caption{Benchmarking different models on the KITTI dataset with different lines.}
    \label{tab:detailed_results_model_sensor}
\end{table*}

==> Supp_Tables/table_pvrcnn_votr_ros_3anchors.tex <==
\begin{table}[t!]
    \centering
    \setlength{\tabcolsep}{1pt}
    \adjustbox{width=\linewidth}{\begin{tabular}{l|c|c|c}
        \toprule
        Model & Waymo  & W $\rightarrow$ K  & W $\rightarrow$ N \\ 
        \hline
        PVRCNN & 71.28 / 62.6  & 58.88 / 13.86  &  31.79 / 20.08 \\ 
        PVRCNN w/ ROS & 65.77 / 57.38 &  &  \\
        PVRCNN 3 Anchors &  &  &  \\
        PVRCNN 3 Anchors w/ ROS  &  &  &  \\ 
        \hline
        VOTR-TSD & 73.87 / 65.2 & 60.06	/ 14.47 & 35.83 / 21.66 \\ 
        VOTR-TSD w/ ROS &   &  &  \\
        VOTR-TSD 3 Anchors &  &  &  \\
        VOTR-TSD 3 Anchors w/ ROS  &  &  &  \\
        
        \bottomrule
    \end{tabular}}
    \caption{Investigating the OOD performance of anchor-based and anchorless detectors on Waymo $\rightarrow$ Kitti and Waymo $\rightarrow$ NuScenes.}
    \label{tab:anchorvslabel}
    \vspace{-1.8em}
\end{table}

==> Supp_Tables/table_pvrcnn_voxel_encoding.tex <==
\begin{table*}[t!]
    \centering
    \adjustbox{width=0.95\textwidth}{\begin{tabular}{c|c|c|cccc|cccc|cccc}
    \hline
        \multirow{2}{*}{NPPV} & \multirow{2}{*}{Task} & \multirow{2}{*}{Class} & \multicolumn{4}{c|}{voxel height: 0.0625m} & \multicolumn{4}{c|}{voxel height: 0.1m} & \multicolumn{4}{c}{voxel height: 0.125m} \\
        ~ & ~ & ~ & Easy & Mod. & Hard & mAP & Easy & Mod. & Hard & mAP & Easy & Mod. & Hard & mAP \\ 
        \hline
        \multirow{9}{*}{4} & \multirow{3}{*}{64} & Car &  91.51  & 82.75  & 80.35  & 84.87  & 91.29  & 80.52  & 79.77  & 83.86  & 91.28  & 82.52  & 80.21  & 84.67  \\ 
        ~ & & Ped  ~ & 66.20  & 59.73  & 55.61  & 60.51  & 68.35  & 59.71  & 55.29  & 61.12  & 66.75  & 59.90  & 55.14  & 60.60  \\ 
        ~ & & Cyc  ~ & 84.22  & 62.81  & 60.11  & 69.05  & 81.42  & 62.41  & 59.72  & 67.85  & 84.90  & 64.03  & 60.08  & 69.67  \\ 
        \cline{2-15} 
        & \multirow{3}{*}{64 $\rightarrow$ 32} & Car ~ & 88.33  & 72.76  & 70.15  & 77.08  & 86.22  & 72.60  & 69.96  & 76.26  & 88.01  & 74.32  & 70.28  & 77.53  \\ 
        ~ & & Ped  ~ & 59.34  & 52.87  & 48.19  & 53.46  & 62.72  & 54.84  & 50.22  & 55.93  & 60.93  & 55.28  & 50.52  & 55.58  \\ 
        ~ & & Cyc  ~ & 65.28  & 41.83  & 39.73  & 48.94  & 65.67  & 42.27  & 40.21  & 49.38  & 70.56  & 45.91  & 43.68  & 53.38  \\ 
        \cline{2-15}
        & \multirow{3}{*}{64 $\rightarrow$ 16} & Car & 69.07  & 48.74  & 44.57  & 54.13  & 66.90  & 46.72  & 43.73  & 52.45  & 68.95  & 48.90  & 44.63  & 54.16  \\ 
        ~ & & Ped  ~ & 25.58  & 22.36  & 20.05  & 22.66  & 32.69  & 28.22  & 24.55  & 28.49  & 27.15  & 25.08  & 22.02  & 24.75  \\ 
        ~ & & Cyc  ~ & 34.02  & 19.61  & 18.01  & 23.88  & 36.04  & 22.04  & 20.08  & 26.06  & 39.24  & 22.61  & 20.61  & 27.49  \\ 
        \midrule
        \multirow{9}{*}{5} & \multirow{3}{*}{64} & Car &  91.66  & 82.73  & 80.30  & 84.90  & 91.26  & 82.51  & 80.22  & 84.66  & 91.61  & 82.72  & 80.38  & 84.90  \\ 
        ~ & & Ped  ~ & 68.06  & 61.28  & 57.04  & 62.13  & 64.51  & 58.45  & 55.40  & 59.45  & 67.66  & 60.47  & 57.40  & 61.84  \\ 
        ~ & & Cyc  ~ & 85.50  & 63.62  & 60.96  & 70.03  & 83.51  & 62.49  & 59.86  & 68.62  & 82.19  & 62.66  & 58.34  & 67.73  \\ 
        \cline{2-15}
        & \multirow{3}{*}{64 $\rightarrow$ 32} & Car ~ & 88.34  & 74.43  & 70.29  & 77.69  & 88.05  & 74.42  & 70.40  & 77.62  & 88.62  & 74.53  & 70.44  & 77.86  \\ 
        ~ & & Ped  ~ & 62.43  & 54.71  & 50.22  & 55.79  & 59.39  & 54.10  & 48.38  & 53.96  & 63.84  & 56.26  & 51.58  & 57.23  \\ 
        ~ & & Cyc  ~ & 66.46  & 43.49  & 41.52  & 50.49  & 64.94  & 44.95  & 41.00  & 50.30  & 67.15  & 44.03  & 41.78  & 50.99  \\ 
        \cline{2-15}
        & \multirow{3}{*}{64 $\rightarrow$ 16} & Car ~ & 68.65  & 48.72  & 44.43  & 53.93  & 68.00  & 49.35  & 44.87  & 54.07  & 71.18  & 49.52  & 45.07  & 55.26  \\ 
        ~ & & Ped  ~ & 24.40  & 22.46  & 19.27  & 22.04  & 30.22  & 27.29  & 23.87  & 27.13  & 37.90  & 33.49  & 29.44  & 33.61  \\ 
        ~ & & Cyc  ~ & 33.02  & 19.44  & 17.69  & 23.38  & 37.42  & 21.68  & 19.98  & 26.36  & 34.71  & 19.41  & 19.31  & 24.48  \\ 
        \midrule
        \multirow{9}{*}{7} & \multirow{3}{*}{64} & Car &  91.98  & 83.20  & 80.68  & 85.29  & 91.49  & 82.56  & 80.24  & 84.76  & 91.22  & 82.37  & 79.88  & 84.49  \\ 
        ~ & & Ped  ~ & 65.61  & 60.02  & 55.75  & 60.46  & 66.41  & 59.77  & 55.51  & 60.56  & 67.08  & 61.13  & 56.72  & 61.64  \\ 
        ~ & & Cyc  ~ & 82.59  & 61.25  & 57.15  & 67.00  & 85.26  & 63.93  & 59.74  & 69.64  & 84.35  & 63.02  & 60.45  & 69.28  \\ 
        \cline{2-15}
        & \multirow{3}{*}{64 $\rightarrow$ 32} & Car ~ & 88.92  & 73.29  & 70.39  & 77.53  & 86.66  & 73.01  & 70.26  & 76.64  & 86.48  & 72.85  & 70.18  & 76.50  \\ 
        ~ & & Ped  ~ & 64.72  & 57.28  & 50.97  & 57.66  & 63.00  & 56.40  & 51.60  & 57.00  & 59.72  & 53.52  & 48.89  & 54.05  \\ 
        ~ & & Cyc  ~ & 61.76  & 39.60  & 37.51  & 46.29  & 67.00  & 44.36  & 42.33  & 51.23  & 69.68  & 46.26  & 44.05  & 53.33  \\ 
        \cline{2-15}
        & \multirow{3}{*}{64 $\rightarrow$ 16} & Car ~ & 68.50  & 47.60  & 42.90  & 53.00  & 67.47  & 47.39  & 42.90  & 52.59  & 67.46  & 48.63  & 44.21  & 53.43  \\ 
        ~ & & Ped  ~ & 33.31  & 28.28  & 25.82  & 29.14  & 33.21  & 28.42  & 26.21  & 29.28  & 28.19  & 25.97  & 22.76  & 25.64  \\ 
        ~ & & Cyc  ~ & 36.29  & 20.37  & 20.11  & 25.59  & 29.15  & 17.40  & 15.50  & 20.68  & 32.81  & 19.16  & 17.54  & 23.17  \\ 
        \midrule
        \multirow{9}{*}{9} & \multirow{3}{*}{64} & Car &  90.94  & 82.27  & 79.98  & 84.40  & 91.48  & 82.45  & 80.08  & 84.67  & 91.45  & 82.55  & 80.18  & 84.73  \\ 
        ~ & & Ped  ~ & 65.81  & 59.39  & 55.18  & 60.12  & 66.31  & 60.82  & 56.43  & 61.19  & 65.06  & 59.11  & 55.08  & 59.75  \\ 
        ~ & & Cyc  ~ & 81.89  & 60.03  & 57.68  & 66.53  & 85.92  & 64.95  & 62.11  & 70.99  & 85.81  & 62.03  & 57.69  & 68.51  \\ 
        \cline{2-15}
        & \multirow{3}{*}{64 $\rightarrow$ 32} & Car ~ & 88.13  & 72.47  & 69.85  & 76.82  & 88.61  & 73.03  & 70.38  & 77.34  & 88.90  & 74.68  & 70.41  & 77.99  \\ 
        ~ & & Ped  ~ & 62.47  & 55.82  & 49.69  & 55.99  & 64.51  & 57.59  & 51.63  & 57.91  & 61.33  & 55.63  & 50.86  & 55.94  \\ 
        ~ & & Cyc  ~ & 67.95  & 44.07  & 41.97  & 51.33  & 70.05  & 44.51  & 42.30  & 52.29  & 72.27  & 47.75  & 43.66  & 54.56  \\ 
        \cline{2-15}
        & \multirow{3}{*}{64 $\rightarrow$ 16} & Car ~ & 68.27  & 46.90  & 42.56  & 52.57  & 68.99  & 49.08  & 44.46  & 54.18  & 69.82  & 49.49  & 45.02  & 54.77  \\ 
        ~ & & Ped  ~ & 26.31  & 22.62  & 19.37  & 22.77  & 34.88  & 30.80  & 27.32  & 31.00  & 30.77  & 27.13  & 23.82  & 27.24  \\ 
        ~ & & Cyc  ~ & 31.56  & 18.04  & 17.65  & 22.42  & 34.52  & 20.80  & 19.42  & 24.91  & 38.28  & 22.21  & 20.40  & 26.96 \\ \hline
    \end{tabular}}
    \caption{PVRCNN-Voxel Encoding}
    \label{tab:pvrcnn_voxel_encoding}
\end{table*}

==> Supp_Tables/table_second_voxel_encoding.tex <==
\begin{table*}[!ht]
    \centering
    \adjustbox{width=0.95\textwidth}{\begin{tabular}{c|c|c|cccc|cccc|cccc}
    \hline
       \multirow{2}{*}{NPPV} & \multirow{2}{*}{Task} & \multirow{2}{*}{Class} & \multicolumn{4}{c|}{voxel height: 0.0625m} & \multicolumn{4}{c|}{voxel height: 0.1m} & \multicolumn{4}{c}{voxel height: 0.125m} \\
        ~ & ~ & ~ & Easy & Mod. & Hard & mAP & Easy & Mod. & Hard & mAP & Easy & Mod. & Hard & mAP \\ 
        \hline 
        \multirow{9}{*}{4} & \multirow{3}{*}{64} & Car/3D & 87.63  & 78.00  & 75.32  & 80.31  & 89.70  & 78.47  & 75.26  & 81.14  & 88.33  & 76.38  & 73.63  & 79.45  \\ 
        ~ & ~ & Ped./3d & 49.82  & 44.80  & 41.45  & 45.36  & 52.75  & 47.70  & 44.03  & 48.16  & 50.10  & 45.34  & 41.74  & 45.73  \\ 
        ~ & ~ & Cyc./3D & 66.89  & 49.20  & 46.85  & 54.31  & 66.92  & 51.51  & 47.65  & 55.36  & 69.13  & 49.82  & 46.20  & 55.05  \\
        \cline{2-15}
        ~ & \multirow{3}{*}{64$\rightarrow$32} & Car/3D & 84.38  & 68.36  & 65.19  & 72.64  & 84.57  & 68.35  & 65.03  & 72.65  & 84.10  & 68.15  & 64.53  & 72.26  \\
        ~ & ~ & Ped./3d & 44.43  & 40.36  & 36.62  & 40.47  & 45.43  & 39.89  & 36.04  & 40.46  & 46.27  & 42.61  & 38.83  & 42.57  \\ 
        ~ & ~ & Cyc./3D & 48.55  & 31.65  & 29.68  & 36.62  & 52.38  & 36.06  & 33.87  & 40.77  & 54.93  & 36.95  & 34.15  & 42.01  \\ 
        \cline{2-15}
        ~ & \multirow{3}{*}{64$\rightarrow$16} & Car/3D & 61.88  & 43.41  & 38.92  & 48.07  & 63.02  & 44.90  & 40.48  & 49.47  & 65.01  & 45.53  & 39.89  & 50.15  \\
        ~ & ~ & Ped./3d & 21.39  & 18.86  & 15.91  & 18.72  & 20.06  & 17.21  & 15.47  & 17.58  & 21.32  & 20.00  & 17.19  & 19.50  \\ 
        ~ & ~ & Cyc./3D & 23.89  & 13.56  & 13.34  & 16.93  & 25.72  & 14.40  & 14.12  & 18.08  & 31.34  & 18.28  & 16.94  & 22.18  \\ 
        \midrule
        \multirow{9}{*}{5} & \multirow{3}{*}{64} & Car/3D & 88.20  & 78.14  & 75.16  & 80.50  & 88.22  & 77.90  & 73.55  & 79.89  & 88.04  & 76.98  & 73.09  & 79.37  \\ 
        ~ & ~ & Ped./3d & 52.27  & 48.06  & 44.56  & 48.30  & 51.00  & 45.77  & 43.31  & 46.69  & 47.30  & 44.01  & 41.02  & 44.11  \\ 
        ~ & ~ & Cyc./3D & 63.09  & 48.39  & 45.81  & 52.43  & 67.46  & 49.32  & 47.02  & 54.60  & 64.62  & 49.69  & 47.04  & 53.78  \\ 
        \cline{2-15}
        ~ & \multirow{3}{*}{64$\rightarrow$32} & Car/3D & 83.38  & 67.55  & 64.21  & 71.71  & 85.21  & 69.94  & 65.35  & 73.50  & 84.10  & 67.92  & 64.56  & 72.19  \\
        ~ & ~ & Ped./3d & 46.01  & 41.95  & 38.39  & 42.11  & 45.22  & 40.96  & 37.15  & 41.11  & 38.25  & 36.26  & 34.17  & 36.23  \\ 
        ~ & ~ & Cyc./3D & 50.72  & 33.39  & 31.66  & 38.59  & 50.68  & 34.17  & 32.44  & 39.10  & 51.93  & 35.11  & 31.98  & 39.68  \\ 
        \cline{2-15}
        ~ & \multirow{3}{*}{64$\rightarrow$16} & Car/3D & 63.26  & 43.92  & 39.24  & 48.81  & 65.76  & 45.63  & 40.74  & 50.71  & 65.26  & 46.14  & 41.23  & 50.88  \\
        ~ & ~ & Ped./3d & 23.15  & 20.47  & 18.54  & 20.72  & 18.56  & 16.51  & 14.81  & 16.63  & 19.86  & 18.87  & 16.52  & 18.41  \\ 
        ~ & ~ & Cyc./3D & 21.70  & 12.58  & 12.37  & 15.55  & 24.46  & 14.30  & 13.99  & 17.58  & 24.24  & 13.22  & 12.78  & 16.75  \\ 
        \midrule
        \multirow{9}{*}{7} & \multirow{3}{*}{64} & Car/3D & 88.16  & 78.52  & 75.73  & 80.80  & 88.26  & 76.07  & 73.45  & 79.26  & 88.38  & 77.82  & 73.68  & 79.96  \\ 
        ~ & ~ & Ped./3d & 53.85  & 48.85  & 45.03  & 49.24  & 54.24  & 49.34  & 45.34  & 49.64  & 49.92  & 45.86  & 42.20  & 45.99  \\ 
        ~ & ~ & Cyc./3D & 69.19  & 53.68  & 49.83  & 57.56  & 69.77  & 50.58  & 47.96  & 56.11  & 70.74  & 51.23  & 47.59  & 56.52  \\ 
        \cline{2-15}
        ~ & \multirow{3}{*}{64$\rightarrow$32} & Car/3D & 84.50  & 68.39  & 65.15  & 72.68  & 84.46  & 68.11  & 63.38  & 71.98  & 84.51  & 68.17  & 64.70  & 72.46  \\
        ~ & ~ & Ped./3d & 46.67  & 41.38  & 37.38  & 41.81  & 47.95  & 42.33  & 38.26  & 42.85  & 46.64  & 42.33  & 38.64  & 42.54  \\ 
        ~ & ~ & Cyc./3D & 56.17  & 37.31  & 34.93  & 42.80  & 52.97  & 35.77  & 33.67  & 40.80  & 55.40  & 35.26  & 33.05  & 41.24  \\ 
        \cline{2-15}
        ~ & \multirow{3}{*}{64$\rightarrow$16} & Car/3D & 61.73  & 43.34  & 38.85  & 47.97  & 64.30  & 44.94  & 39.47  & 49.57  & 64.67  & 45.68  & 40.79  & 50.38  \\
        ~ & ~ & Ped./3d & 19.40  & 17.58  & 14.96  & 17.31  & 19.35  & 17.82  & 15.30  & 17.49  & 19.57  & 18.61  & 16.03  & 18.07  \\ 
        ~ & ~ & Cyc./3D & 26.86  & 15.16  & 13.57  & 18.53  & 27.37  & 15.99  & 14.73  & 19.36  & 26.26  & 14.90  & 14.75  & 18.64  \\
        \midrule
        \multirow{9}{*}{9} & \multirow{3}{*}{64} & Car/3D & 86.47  & 74.95  & 72.47  & 77.96  & 88.40  & 77.85  & 73.43  & 79.89  & 87.55  & 75.74  & 73.13  & 78.80  \\ 
        ~ & ~ & Ped./3d & 55.72  & 50.13  & 45.92  & 50.59  & 52.73  & 47.74  & 44.32  & 48.26  & 55.09  & 49.26  & 45.41  & 49.92  \\ 
        ~ & ~ & Cyc./3D & 68.48  & 53.09  & 49.13  & 56.90  & 70.03  & 51.47  & 47.62  & 56.37  & 66.32  & 49.50  & 46.79  & 54.21  \\
        \cline{2-15}
        ~ & \multirow{3}{*}{64$\rightarrow$32} & Car/3D & 81.04  & 65.00  & 62.06  & 69.37  & 84.65  & 67.89  & 64.47  & 72.34  & 83.34  & 67.50  & 62.96  & 71.27  \\
        ~ & ~ & Ped./3d & 49.50  & 43.23  & 39.19  & 43.97  & 47.03  & 42.50  & 38.14  & 42.56  & 46.83  & 42.69  & 38.76  & 42.76  \\ 
        ~ & ~ & Cyc./3D & 51.60  & 34.10  & 32.14  & 39.28  & 52.15  & 34.60  & 32.68  & 39.81  & 50.10  & 34.77  & 32.12  & 39.00  \\
        \cline{2-15}
        ~ & \multirow{3}{*}{64$\rightarrow$16} & Car/3D & 58.60  & 40.70  & 36.50  & 45.27  & 64.38  & 44.07  & 39.33  & 49.26  & 65.18  & 44.47  & 39.56  & 49.74  \\ 
        ~ & ~ & Ped./3d & 20.68  & 17.97  & 14.83  & 17.83  & 17.63  & 15.45  & 13.71  & 15.60  & 20.52  & 18.61  & 16.76  & 18.63  \\ 
        ~ & ~ & Cyc./3D & 21.00  & 11.91  & 11.96  & 14.96  & 24.87  & 14.78  & 13.94  & 17.86  & 25.53  & 14.84  & 13.60  & 17.99 \\ \hline
    \end{tabular}}
    \caption{Second: Voxel Encoding}
    \label{tab:second_voxel_encoding}
\end{table*}

==> Supp_Tables/table_votr_voxel_encoding.tex <==
\begin{table*}[t!]
    \centering
    \adjustbox{width=0.90\textwidth}{\begin{tabular}{c|c|c|cccc|cccc|cccc}
    \hline
        \multirow{2}{*}{NPPV} & \multirow{2}{*}{Task} & \multirow{2}{*}{Class} &  \multicolumn{4}{c|}{voxel height: $0.0625m$} & \multicolumn{4}{c|}{voxel height: $0.1m$} & \multicolumn{4}{c}{voxel height: $0.125m$} \\ 
        ~ &~ &~ & Easy & Mod. & Hard & mAP & Easy & Mod. & Hard & mAP & Easy & Mod. & Hard & mAP \\ 
        \midrule
        \multirow{9}{*}{4} & \multirow{3}{*}{64} & Car & 91.50  & 82.93  & 80.35  & 84.93  & 89.08  & 80.28  & 77.81  & 82.39  & 88.96  & 79.62  & 77.11  & 81.90  \\ 
        & ~ & Ped. & 59.09  & 55.87  & 51.31  & 55.42  & 53.98  & 50.30  & 47.29  & 50.52  & 62.75  & 57.15  & 53.17  & 57.69  \\ 
        & ~ & Cyc. & 75.29  & 55.41  & 53.00  & 61.23  & 79.77  & 60.05  & 56.02  & 65.28  & 74.82  & 56.68  & 54.06  & 61.85  \\ 
        \cline{2-15}
        & \multirow{3}{*}{64 $\rightarrow 32$} & Car &  86.67  & 74.85  & 72.18  & 77.90  & 85.88  & 72.24  & 69.58  & 75.90  & 86.24  & 72.18  & 69.42  & 75.95  \\ 
        &~ & Ped. &  56.01  & 51.08  & 46.97  & 51.36  & 50.33  & 46.72  & 43.26  & 46.77  & 62.09  & 56.40  & 50.78  & 56.42  \\ 
       & ~ & Cyc. &  65.91  & 43.37  & 41.15  & 50.15  & 61.79  & 42.72  & 40.40  & 48.31  & 68.12  & 45.55  & 43.27  & 52.31  \\ 
        \cline{2-15}
        & \multirow{3}{*}{64 $\rightarrow$ 16} & Car &  71.64  & 53.14  & 48.75  & 57.84  & 68.83  & 50.45  & 45.97  & 55.08  & 72.03  & 51.54  & 47.08  & 56.88  \\ 
        &~ & Ped. &  27.76  & 24.85  & 22.97  & 25.19  & 29.17  & 25.50  & 23.64  & 26.10  & 41.22  & 36.71  & 32.98  & 36.97  \\ 
       & ~ & Cyc. &  31.66  & 18.99  & 17.22  & 22.62  & 33.48  & 20.15  & 18.53  & 24.06  & 41.68  & 23.11  & 22.93  & 29.24  \\ 
        \midrule
        \multirow{9}{*}{5} & \multirow{3}{*}{64} & Car &  91.12  & 82.24  & 79.98  & 84.45  & 88.99  & 82.09  & 79.90  & 83.66  & 89.45  & 82.33  & 80.11  & 83.96  \\ 
        &~ & Ped. &  55.91  & 53.31  & 49.64  & 52.95  & 58.83  & 55.00  & 51.63  & 55.15  & 60.59  & 56.57  & 53.26  & 56.81  \\ 
       & ~ & Cyc. &  70.13  & 54.09  & 51.50  & 58.57  & 75.67  & 58.28  & 54.37  & 62.78  & 75.17  & 56.87  & 54.27  & 62.11  \\ 
        \cline{2-15}
        & \multirow{3}{*}{64 $\rightarrow$ 32} & Car &  86.21  & 74.68  & 72.12  & 77.67  & 86.15  & 72.66  & 70.07  & 76.29  & 86.42  & 74.64  & 72.18  & 77.75  \\ 
        &~ & Ped. &  51.19  & 47.66  & 44.29  & 47.72  & 54.26  & 49.34  & 45.73  & 49.78  & 57.15  & 52.61  & 48.72  & 52.83  \\ 
       & ~ & Cyc. &  57.81  & 39.35  & 37.08  & 44.75  & 64.29  & 43.62  & 41.38  & 49.76  & 65.04  & 45.50  & 43.30  & 51.28  \\ 
        \cline{2-15}
        & \multirow{3}{*}{64 $\rightarrow$ 16} & Car &  71.64  & 53.18  & 48.80  & 57.87  & 69.28  & 50.97  & 46.59  & 55.61  & 71.73  & 53.28  & 48.97  & 57.99  \\ 
        &~ & Ped. &  27.23  & 23.26  & 20.25  & 23.58  & 23.92  & 21.55  & 19.66  & 21.71  & 32.53  & 30.22  & 26.81  & 29.85  \\ 
       & ~ & Cyc. &  29.64  & 17.72  & 17.62  & 21.66  & 34.62  & 19.33  & 19.19  & 24.38  & 37.77  & 21.13  & 20.80  & 26.57  \\ 
        \midrule
        \multirow{9}{*}{7} & \multirow{3}{*}{64} & Car & 88.20  & 79.57  & 77.18  & 81.65  & 91.48  & 82.77  & 80.34  & 84.86  & 88.38  & 79.61  & 76.94  & 81.64  \\ 
         &~ & Ped. &  50.21  & 47.77  & 44.09  & 47.35  & 57.19  & 55.30  & 52.60  & 55.03  & 57.41  & 53.41  & 50.21  & 53.67  \\ 
       & ~ & Cyc. &  73.45  & 55.91  & 53.37  & 60.91  & 72.43  & 56.46  & 52.69  & 60.53  & 64.51  & 50.41  & 48.21  & 54.38  \\ 
        \cline{2-15}
        & \multirow{3}{*}{64 $\rightarrow$ 32} & Car &  85.13  & 71.74  & 69.11  & 75.32  & 88.25  & 74.93  & 72.34  & 78.51  & 85.39  & 71.67  & 68.93  & 75.33  \\ 
         &~ & Ped. &  49.36  & 45.42  & 42.13  & 45.64  & 55.51  & 51.36  & 47.69  & 51.52  & 59.26  & 54.31  & 49.35  & 54.31  \\ 
       & ~ & Cyc. &  62.05  & 43.22  & 41.12  & 48.80  & 62.94  & 43.78  & 40.29  & 49.00  & 60.85  & 42.01  & 41.47  & 48.11  \\ 
        \cline{2-15}
        & \multirow{3}{*}{64 $\rightarrow$ 16} & Car &  69.79  & 50.53  & 47.71  & 56.01  & 70.32  & 51.39  & 48.42  & 56.71  & 69.80  & 52.14  & 47.93  & 56.62  \\ 
         &~ & Ped. &  29.78  & 27.05  & 23.76  & 26.86  & 30.27  & 27.82  & 25.60  & 27.90  & 31.97  & 28.99  & 25.60  & 28.85  \\ 
       & ~ & Cyc. &  37.55  & 22.29  & 20.77  & 26.87  & 34.41  & 19.98  & 18.57  & 24.32  & 39.69  & 22.73  & 22.41  & 28.28  \\ 
        \midrule
         \multirow{9}{*}{9} & \multirow{3}{*}{64} & Car &88.81  & 80.03  & 77.46  & 82.10  & 88.84  & 80.33  & 77.57  & 82.25  & 89.40  & 80.31  & 77.80  & 82.50  \\ 
         &~ & Ped. &  55.46  & 52.45  & 48.12  & 52.01  & 49.33  & 46.05  & 43.83  & 46.40  & 52.97  & 50.75  & 48.27  & 50.66  \\ 
       & ~ & Cyc. &  75.44  & 56.87  & 52.98  & 61.76  & 76.33  & 55.53  & 52.94  & 61.60  & 72.30  & 54.31  & 51.74  & 59.45  \\ 
        \cline{2-15}
        & \multirow{3}{*}{64 $\rightarrow$ 32} & Car &  85.96  & 71.90  & 69.23  & 75.70  & 86.00  & 72.15  & 69.30  & 75.82  & 86.38  & 72.59  & 69.88  & 76.28  \\ 
         &~ & Ped. &  51.32  & 47.20  & 43.65  & 47.39  & 45.25  & 42.32  & 40.62  & 42.73  & 56.36  & 51.50  & 47.69  & 51.85  \\ 
       & ~ & Cyc. &  66.44  & 44.74  & 40.94  & 50.71  & 63.45  & 45.44  & 41.76  & 50.22  & 63.42  & 44.47  & 42.37  & 50.09  \\ 
        \cline{2-15}
        & \multirow{3}{*}{64 $\rightarrow$ 16} & Car &  68.95  & 50.74  & 47.82  & 55.84  & 70.09  & 50.82  & 46.35  & 55.75  & 69.28  & 50.69  & 46.27  & 55.42  \\ 
         &~ & Ped. &  26.68  & 23.92  & 20.98  & 23.86  & 20.41  & 19.52  & 18.09  & 19.34  & 29.50  & 25.90  & 24.14  & 26.51  \\ 
       & ~ & Cyc. &  38.16  & 22.77  & 20.97  & 27.30  & 37.13  & 21.55  & 19.69  & 26.12  & 44.46  & 25.49  & 25.43  & 31.79 \\ \hline
    \end{tabular}}
    \caption{ VOTR-TSD: Voxel Encoding}
    \label{tab:votr_voxel_encoding}
\end{table*}

==> Supp_Tables/table_weather_voxel_size.tex <==
\begin{table*}[h!]
\centering
\renewcommand\arraystretch{1.2}
\setlength{\tabcolsep}{2pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{ccccccccccccc}
\toprule
& \multicolumn{6}{c|}{Source Domain - Waymo} & \multicolumn{6}{c}{Target Domain - Kirk} \\ \hline
\multicolumn{1}{c|}{} & \multicolumn{3}{c|}{Veh. 3D-AP}& \multicolumn{3}{c|}{Ped. 3D-AP}& \multicolumn{3}{c|}{Veh. 3D-AP}& \multicolumn{3}{c}{Ped. 3D-AP}\\
\multicolumn{1}{c|}{\multirow{-2}{*}{Voxel Size}} & LEVEL\_1& LEVEL\_2& \multicolumn{1}{c|}{mAP} & LEVEL\_1& LEVEL\_2& \multicolumn{1}{c|}{mAP} & LEVEL\_1& LEVEL\_2& \multicolumn{1}{c|}{mAP} & LEVEL\_1& LEVEL\_2& mAP \\ \hline
\multicolumn{1}{c|}{(0.1, 0.1, 0.1)}& {\color[HTML]{FF0000} \textbf{75.53}} & {\color[HTML]{FF0000} \textbf{67.00}} & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{71.27}}} & {\color[HTML]{FF0000} \textbf{72.71}} & \second{63.71}& \multicolumn{1}{c|}{\second{68.21}}& {\color[HTML]{FF0000} \textbf{60.60}} & {\color[HTML]{FF0000} \textbf{50.96}} & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{55.78}}} & \second{27.90}& \second{19.56}& \second{23.73}\\
\multicolumn{1}{c|}{(0.1, 0.1, 0.15)} & \second{75.26}& \second{66.75}& \multicolumn{1}{c|}{\second{71.01}}& {\color[HTML]{FF0000} \textbf{72.71}} & {\color[HTML]{FF0000} \textbf{63.74}} & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{68.23}}} & \second{59.77}& \second{50.26}& \multicolumn{1}{c|}{\second{55.02}}& {\color[HTML]{FF0000} \textbf{28.04}} & {\color[HTML]{FF0000} \textbf{19.65}} & {\color[HTML]{FF0000} \textbf{23.85}} \\
\multicolumn{1}{c|}{(0.15, 0.1, 0.15)}& 75.22 & \second{66.75}& \multicolumn{1}{c|}{70.99} & 70.89 & 61.93 & \multicolumn{1}{c|}{66.41} & 59.71 & 50.10 & \multicolumn{1}{c|}{54.91} & 25.79 & 18.12 & 21.96 \\
\multicolumn{1}{c|}{(0.1, 0.1, 0.175)}& 74.51 & 65.99 & \multicolumn{1}{c|}{70.25} & 71.79 & 62.80 & \multicolumn{1}{c|}{67.30} & 58.96 & 49.52 & \multicolumn{1}{c|}{54.24} & 25.07 & 17.60 & 21.34 \\
\multicolumn{1}{c|}{(0.1, 0.1, 0.2)}& 73.18 & 64.62 & \multicolumn{1}{c|}{68.90} & 69.08 & 59.99 & \multicolumn{1}{c|}{64.54} & 56.93 & 47.50 & \multicolumn{1}{c|}{52.22} & 21.85 & 15.34 & 18.60 \\ \hline
\end{tabular}}
\caption{Voxel encoding of PVRCNN in Waymo datasets. The best results are indicated in red and the second-best results are indicated in blue.}
\label{weather_voxel_encoding}
\vspace{-1em}
\end{table*}

==> Tables/anchor_size.tex <==
\begin{table}[t!]
    \centering
    \setlength{\tabcolsep}{2pt}
    \adjustbox{width=\linewidth}{\begin{tabular}{l|l|c|c}
    \hline
        Trained Anchor  & Test Anchor & Waymo $\rightarrow$ KITTI & Waymo $\rightarrow$ nuScenes \\ 
        \hline
        \multirow{3}{*}{Default Waymo} & Training anchor [4.2, 2.0, 1.6] & 54.90/16.41 & 31.69/18.69 \\ 
        ~ & Best on nuScenes [4.2, 1.8, 1.65] & 77.13/41.13 & \textbf{31.80}/\textbf{21.31} \\ 
        ~ & Best on KITTI [3.8, 1.7, 1.50] & 81.13/66.81 & 27.18/9.40 \\ 
        ~ & MOS KITTI [3.89, 1.62, 1.53] & \textbf{81.31}/\textbf{68.94} & 26.02/9.74 \\ 
        \multirow{-5}{*}{[4.2, 2.0, 1.6]} & MOS nuScenes [4.51, 1.96, 1.73] & 27.18/0.27 & 29.94/12.88 \\ 
        \midrule
        \multirow{3}{*}{Default KITTI} & Training anchor [3.9, 1.6, 1.56] & 52.80/11.06 & 31.59/18.49 \\ 
        ~ & Best on nuScenes [3.8, 1.5 , 1.6] & 76.78/32.31 & \textbf{32.0}/\textbf{21.17} \\ 
        ~ & Best on KITTI [3.6, 1.3, 1.5] & \textbf{81.38}/\textbf{68.19} & 26.05/12.35 \\ 
        ~ & MOS KITTI [3.89, 1.62, 1.53] & 48.35/11.67 & 31.34/17.10 \\ 
         \multirow{-5}{*}{[3.9, 1.6, 1.56]} & MOS nuScenes [4.51, 1.96, 1.73] & 0.0/0.0 & 4.55/0.70 \\ 
         \hline
         \hline
         \multicolumn{2}{l|}{ST3D$^{*}$~\cite{st3d}} & 82.19/61.83  & 35.92/20.19 \\ 
         \multicolumn{2}{l|}{ST3D++$^{*}$~\cite{st3d++}} & 80.78/65.64  & 35.73/20.90 \\
         \multicolumn{2}{l|}{ST3D++$^{*}$ w/ SN ~\cite{st3d++}} & \textbf{86.47}/\textbf{74.61}  & \textbf{36.65}/\textbf{22.01} \\
         \bottomrule
    \end{tabular}}
    \caption{Evaluation of different anchor sizes at test-time on W$\rightarrow$K car benchmark. Three training experiments using SECOND are performed, each with a different anchor size. Using the same size at test-time results in a poor performance, but a very high peak can be obtained by going for lower anchor sizes.}
    \label{tab:anchor_size}
    \vspace{-1.5em}
\end{table}

%Changing the test-time anchor size solely can significantly yield improvement gains.

==> Tables/aug_env.tex <==
\begin{table}[t!]
    \centering
    \setlength{\tabcolsep}{2pt}
    \adjustbox{width=\linewidth}{\begin{tabular}{cccccc}
    \hline
        Dataset & Model & No AUG & GT & LD & SA \\ \hline
        \multirow{2}{*}{Waymo} & PVRCNN & 71.71/62.95 & 73.0/64.26 & 72.02/63.33 & 72.63/63.89 \\ 
        ~ & VOTR & 73.84/65.18 & 73.68/65.06 & 73.47/64.80 & \textbf{73.98}/\textbf{65.31} \\ 
        \midrule
        \multirow{2}{*}{Waymo $\rightarrow$KITTI} & PVRCNN & 58.88/13.86 & 59.38/12.97 & 60.2/13.93 & 61.43/13.99 \\ 
        ~ & VOTR & 60.06/14.47 & \textbf{64.2}/\textbf{18.7} & 63.24/14.36 & 62.49/15.12 \\ 
        \midrule
        \multirow{2}{*}{Waymo $\rightarrow$nuScenes} & PVRCNN & 31.79/20.08 & 33.74/20.07 & 39.68/23.98 & 36.18/23.59 \\ 
        ~ & VOTR & 35.83/21.66 & 35.28/20.93 & \textbf{42.71}/\textbf{24.94} & 38.65/23.87\\ \hline
    \end{tabular}}
    \caption{Effect of data augmentation strategies on the OOD performance of VOTR-TSD and PVRCNN across different geographical locations. We bold the best results on each dataset.}
    \label{tab:aug_env}
    \vspace{-1.5em}
\end{table}

==> Tables/benchmark.tex <==
\begin{table*}[!ht]
    \centering
    \renewcommand\arraystretch{1}
    %\setlength{\tabcolsep}{10pt}
    \adjustbox{width=\linewidth}{
    \begin{tabular}{c|c|c|cc|cc|cc|cc|cc|cc|cc}
    \hline
    \toprule
        \multirow{2}{*}{Features} & \multirow{2}{*}{Architecture} & \multirow{2}{*}{Method} & \multicolumn{2}{c|}{K64$\rightarrow$K32 (R)} & \multicolumn{2}{c|}{K64$\rightarrow$K16 (R)} & \multicolumn{2}{c|}{W$\rightarrow$K (G)}  & \multicolumn{2}{c|}{W$\rightarrow$N (G+R)} & \multicolumn{2}{c|}{W$\rightarrow$Kr (W)} & \multicolumn{2}{c|}{N$\rightarrow$K (G+R)} & \multicolumn{2}{c}{Mean} \\
        ~ & ~ & ~ & Car & Ped & Car & Ped & Car & Ped & Car & Ped & Car & Ped & Car & Ped & Car & Ped \\
        \midrule
        Point & MLP & PointRCNN & 74.70 & 51.86 & 51.74 & 21.03 & 5.04 & 28.22 & 12.00 & 3.92 & 19.24 & 5.86 & 13.81 & 25.31 & 29.42 & 22.7 \\ \midrule
        Voxel & Conv & PointPillars & 70.48 & 35.81 & 53.16 & 20.5 & 12.75 & 48.34 & 20.90 & 5.45 & 46.77 & 13.79 & 0.04 & 0.00 & 34.01 & 20.65 \\ 
        ~ & Conv & Second & 73.50 & 41.11 & 50.71 & 16.63 & 9.91 & 41.39 & 17.84 & 4.44 & 46.04 & 14.97 & 6.36 & 13.43 & 34.06 & 22.0 \\ 
        ~ & Conv & VoxelRCNN & 76.96 & \textbf{56.71} & \textbf{56.11} & \textbf{27.24} & \textbf{20.09} & \textbf{55.33} & 19.71 & 0.05 & 52.18 & 20.7 & 7.48 & 20.96 & 38.75 & \textbf{30.16}  \\ 
        ~ & ViT & VOTR-VoxelRCNN & 76.05 & 51.62 & 55.7 & 24.55 & 21.34 & 29.96 & 15.34 & 0.02 & 49.21 & 15.81 & 19.26 & \textbf{26.82} & 39.48 & 24.80 \\ \midrule 
        Hybrid & Conv & CenterPoint & 71.18 & 42.71 & 52.8 & 15.11 & 13.78 & 53.39 & 19.05 & 5.63 & 50.23 & \textbf{30.72} & 8.96 & 19.94 & 36.00 & 27.92 \\ 
        ~ & Conv & PVRCNN Centerhead & 71.39 & 44.64 & 44.24 & 15.39 & 15.06 & 52.47 & 20.59 & 6.84 & \textbf{52.79} & 29.02 & \textbf{28.52} & 21.67 & 38.76 & 28.34  \\ 
        ~ & Conv & PVRCNN &\textbf{ 77.62} & 53.96 & 54.07 & 27.13 & 16.61 & 50.22 & 20.36 & 5.79 & 54.34 & 25.79 & 10.46 & 17.46 & 38.91 & 30.06 \\ 
        ~ & ViT & VOTR-TSD & 76.29 & 49.78 & 55.61 & 21.71 & 15.75 & 46.19 & \textbf{21.32} & \textbf{7.00} & 52.52 & 26.56 & 26.26 & 26.56 & \textbf{41.29} & 29.63 \\ \bottomrule
    \end{tabular}}
    \caption{Evaluation of different architectures on six DA benchmarks. Beside each benchmark, we denote whether it is mainly caused by a resolution (R), weather (W) or geographical location (G) discrepancy. Voxel Transformers and hybrid representations are found to be, on average, more resilient on the car and pedestrian classes.}
    \label{tab:benchmark}
\end{table*}

%Should we add cyclist in this benchmark ? 

==> Tables/weather_models.tex <==
\begin{table}[t!]
    \centering
    \setlength{\tabcolsep}{3pt}
    \renewcommand\arraystretch{0.95}
    \adjustbox{width=\linewidth}{\begin{tabular}{c|cc|cc|cc}
    \toprule
        \multirow{2}{*}{Models} & \multicolumn{2}{c|}{Waymo} & \multicolumn{2}{c|}{Waymo $\rightarrow$ Kirk} & \multicolumn{2}{c}{Oracle Kirk} \\ 
        & Vehicle & Ped & Vehicle & Ped & Vehicle & Ped \\
        \midrule
        PointRCNN & 29.40 & 7.79 & 19.24 & 5.86 & 23.14 & 2.64 \\ 
        \midrule
        PointPillar & 59.80 & 50.51 & 46.77 & 13.79 & 48.87 & 3.53 \\ 
        Second & 60.96 & 49.59 & 46.04 & 14.97 & 47.83 & 8.35 \\ 
        CenterPoint & 64.67 & \best{65.43} & 50.23 & \best{30.72} & 50.87 & \best{23.33} \\ 
        VoxelRCNN & 65.82 & 54.07 & 52.18 & 20.7 & \second{57.09} & 12.31 \\
        VOTR-VoxelRCNN & 63.32 & 47.31 & 49.21 & 15.81 & N/A & N/A \\    
        \midrule
        PVRCNN & \second{68.3} & 61.79 & \second{54.34} & 25.79 & \best{58.03} & 16.11 \\
        PVRCNN-Centerhead & 67.39 & \second{64.79} & 52.79 & \second{29.02} & 56.85 & \second{18.37} \\ 
        VOTR-TSD & \best{70.26} & 63.42 & \best{55.20} & 26.56 & N/A & N/A \\ 
        \bottomrule
    \end{tabular}}
    \caption{Benchmarking of 3D detectors on Waymo $\rightarrow$ Kirk. The {\best{best}} and {\second{second-best}} results are color-coded to show best-performing models. VOTR-TSD does not converge on Kirkland.}
    \label{tab:weather_models}
    \vspace{-0.5em}
\end{table}

==> draft.tex <==
\begin{table*}[!ht]
    \centering
    \renewcommand\arraystretch{1}
    %\setlength{\tabcolsep}{10pt}
    \adjustbox{width=\linewidth}{
    \begin{tabular}{c|c|c|cc|cc|cc|cc|cc|cc|cc}
    \hline
    \toprule
        \multirow{2}{*}{Features} & \multirow{2}{*}{Architecture} & \multirow{2}{*}{Method} & \multicolumn{2}{c|}{K64$\rightarrow$K32 (R)} & \multicolumn{2}{c|}{K64$\rightarrow$K16 (R)} & \multicolumn{2}{c|}{W$\rightarrow$K (G)}  & \multicolumn{2}{c|}{W$\rightarrow$N (G+R)} & \multicolumn{2}{c|}{W$\rightarrow$Kr (W)} & \multicolumn{2}{c|}{N$\rightarrow$K (G+R)} & \multicolumn{2}{c}{Mean} \\
        ~ & ~ & ~ & Car & Ped & Car & Ped & Car & Ped & Car & Ped & Car & Ped & Car & Ped & Car & Ped \\
        \midrule
        Point & MLP & PointRCNN & 74.70 & 51.86 & 51.74 & 21.07 & 5.38 & 29.8 & 12.0 & 3.91 & 19.24 & 5.86 & 13.64 & 25.31 & 29.77 & 22.60 \\ \midrule
        Voxel & Conv & PointPillars & 70.48 & 35.81 & 53.16 & 20.50 & 12.74 & 48.35 & 21.01 & 5.45 & 46.77 & 13.79 & 0.04 & 0.0 & 34.03 & 20.65 \\ 
        ~ & Conv & SECOND & 73.5 & 41.11 & 50.71 & 16.63 & 16.41 & 41.83 & 18.69 & 4.44 & 46.035 & 14.97 & 4.97 & 13.43 & 35.05 & 22.07 \\ 
        ~ & Conv & VoxelRCNN & \textbf{76.96} & \textbf{56.71} & \textbf{56.11} & \textbf{27.24} & \textbf{18.28} & \textbf{55.34} & 19.46 & 0.045 & 52.175 & 20.7 & 8.74 & 20.96 & 38.62 & 30.16 \\ 
        ~ & ViT & VOTR-VoxelRCNNhead & 76.05 & 51.62 & 55.7 & 24.55 & 17.53 & ~ & 19.39 & ~ & 49.205 & 15.81 & 18.47 & 26.82 & 39.39 & 29.7 \\ \midrule 
        Hybrid & Conv & CenterPoint & 71.18 & 42.71 & 52.80 & 15.11 & 11.86 & 53.39 & 18.35 & 5.63 & 50.225 & 30.72 & 16.50 & 19.94 & 36.82 & 27.92 \\ 
        ~ & Conv & PVRCNN Centerhead & 71.39 & 44.64 & 44.24 & 15.39 & 10.07 & 52.48 & 19.79 & 6.84 & 52.785 & 29.02 & 20.062 & 21.67 & 36.39 & 28.34 \\ 
        ~ & Conv & PVRCNN & 77.62 & 53.96 & 54.07 & 27.13 & 13.86 & 50.22 & 20.08 & 5.79 & \textbf{54.34} & 25.79 & 14.83 & 17.46 & 39.13 & 30.05 \\ 
        ~ & ViT & VOTR-TSD & 76.29 & 49.78 & 55.61 & 21.71 & 14.46 & ~ & \textbf{21.66} & ~ & 52.52 & \textbf{26.56} & \textbf{24.7478} & \textbf{26.56} & \textbf{40.88} & \textbf{31.15} \\ \bottomrule
    \end{tabular}}
    \caption{Evaluation of different architectures on six DA benchmarks. Beside each benchmark, we denote whether it is mainly caused by a resolution (R), weather (W) or geographical location (G) discrepancy. Voxel Transformers and hybrid representations are found to be on average more resilient on the car and pedestrian classes.}
    \label{tab:benchmark}
\end{table*}
